Efficient Multivariate Time Series Forecasting via Calibrated Language Models with Privileged Knowledge Distillation

Multivariate time series forecasting (MTSF) endeavors to predict future observations given historical data, playing a crucial role in time series data management systems. With advancements in large language models (LLMs), recent studies employ textual prompt tuning to infuse the knowledge of LLMs into MTSF. However, the deployment of LLMs often suffers from low efficiency during the inference phase. To address this problem, we introduce TimeKD, an efficient MTSF framework that leverages the calibrated language models and privileged knowledge distillation. TimeKD aims to generate high-quality future representations from the proposed cross-modality teacher model and cultivate an effective student model. The cross-modality teacher model adopts calibrated language models (CLMs) with ground truth prompts, motivated by the paradigm of Learning Under Privileged Information (LUPI). In addition, we design a subtractive cross attention (SCA) mechanism to refine these representations. To cultivate an effective student model, we propose an innovative privileged knowledge distillation (PKD) mechanism including correlation and feature distillation. PKD enables the student to replicate the teacher's behavior while minimizing their output discrepancy. Extensive experiments on real data offer insight into the effectiveness, efficiency, and scalability of the proposed TimeKD.

==> sections/sec1_intro.tex <==
\section{Introduction}
\label{sec:intro}

% ========================================
% Paragraph 1
% Background
% ========================================
Multivariate time series forecasting (MTSF) plays an important role in time series data management systems, which aims to learn intricate temporal dynamics given historical time series~\cite{zha2024scaling, chang2024timedrl,shao2024exploring}. % to predict future values. 
The proliferation of edge devices generates a large amount of time series in various domains~\cite{kieu2022anomaly,campos2023lightts,ding2024tsddiscover}, facilitating a range of real-world applications, e.g., investment strategies~\cite{zheng2024cross}, weather preparedness~\cite{fang2023spatio}, urban planning~\cite{sun2024urban}, and energy management~\cite{guo2024data}.

% ========================================
% Paragraph 2-3
% Existing MTSF models and limitations
% 1. Small models have less params and data -> weak generalization ability
% 2. large models on multivariate time series
% ========================================

Existing methods for MTSF, i.e., Transformer-based methods~\cite{Yuqietal-2023-PatchTST,DBLP:journals/corr/abs-2310-06625}, linear methods~\cite{Zeng2022AreTE}, and convolutional methods~\cite{wu2023timesnet}, often face limitations due to a restricted number of learnable parameters and dependency on small-scale training datasets~\cite{liutimer}. These constraints lead to weak generalization capabilities and inconsistent performance on multivariate time series tasks. Recent advancements have begun integrating pre-trained large language models (LLMs) into time series forecasting~\cite{DBLP:conf/nips/ZhouNW0023, chang2023llm4ts, sun2023test,xue2023promptcast}. By leveraging the robust embeddings of LLMs~\cite{DBLP:conf/kdd/LiangWNJ0SPW24}, which are trained on extensive language corpora, these methods enhance the representation of multivariate time series, enabling more effective forecasting.
% ========================================
% Paragraph 4
% LLM KD for MTSF (Related Work B)
% ========================================

Most recent LLM-based forecasting methods utilize multimodal inputs containing both numerical time series information and textual information. Some works directly take pure text information as one of the modal inputs~\cite{jia2024gpt4mts, liu2024unitime} while others align the time series input with the time series-textual embedding of LLMs~\cite{cao2023tempo, DBLP:journals/corr/abs-2406-01638, jin2023time}. However, the general text embeddings from LLMs may not correlate well with time series data distribution. Moreover, the existing LLM-based forecasting methods suffer from high computational costs during test process.

%However, the domain gap between language and time series data makes it difficult for historical data of time series to directly learn ground truth data distribution. The mapping from historical data to ground truth remains implicit. This raises a question:\textit{ How can we explicitly model the transformation from historical data to ground truth for improved forecasting?}

% \begin{figure}[t]
%     \begin{centering}	
%     \includegraphics[width=0.45\textwidth]{Figs/LUPI.pdf}
%         \caption{Learning Under Privileged Information (LUPI) paradigm for time series forecasting. Leveraging \textbf{ground truth as privileged information} that is only available during the training process.}
%         \label{fig:intro}
%     \end{centering}
% \end{figure}

% \begin{figure}[t]
%     \begin{centering}	
%     \includegraphics[width=0.5\textwidth]{Figs/Intro.pdf}
%         \caption{Comparison of inputs in large language model-based knowledge distillation. (a) Existing approaches use textual modality with historical data or text instructions. (b) Our inputs are in the Learning Under Privileged Information (LUPI) paradigm, where ground truth is treated as privileged information accessible only during the training phase.}
%         \label{fig:intro}
%     \end{centering}
% \end{figure}

To this end, we leverage the Learning Under Privileged Information (LUPI)~\cite{DBLP:journals/corr/Lopez-PazBSV15} paradigm, which consists of a privileged text modality branch and a time series modality branch. We utilize the ground truth texts as the input for the text modality branch to provide privileged information for historical data explicitly for modeling the data transformation from the past to the future. To leverage the privileged information but not explicitly anticipate it, we introduce a Knowledge Distillation (KD) based framework for time series forecasting. The privileged information is only available during the training process. In the test process, only observed time series is used for forecasting. While leveraging large language models (LLMs) and the Learning Under Privileged Information (LUPI) paradigm presents promising directions for MTSF, several critical challenges are expected to be addressed to ensure effectiveness and efficiency. 

%Although LLMs are effective for dealing with text data, their computational overhead cannot be ignored. Existing works reduce this cost by extracting the last token embedding generated by the LLM. We adopt a similar approach and eliminate the LLM during the testing phase through knowledge distillation. We propose a privileged knowledge distillation framework to transfer this privileged information to the forecasting model. In this framework, the LLM processes historical data and ground truth to generate embeddings and attention distributions. These privileged embeddings are then distilled into a lightweight model, which learns to replicate the teacher's enriched representations using only historical data.

% ========================================
% Paragraph 5
% Challenges of LLM KD for MTFS
% 1. Good Teacher and privileged knowledge
% 2. How to teach
% 3. Efficiency
% ========================================

\textbf{Challenge I: How to train bridge the domain gap between text and time series modalities?} The inherent differences between language and time series data, such as sequential dependencies in time series versus the semantic relationships in language pose challenges. Directly applying LLMs to time series data often leads to ineffective representations, as the embeddings generated by the LLM may fail to capture the temporal dynamics and cross-variable correlations inherent in multivariate time series.

\textbf{Challenge II: How to solve the data entanglement issues between text and time series data?} The attention mechanisms in large language models (LLMs), while effective for capturing relationships in language data, can inadvertently lead to data entanglement when applied to multimodal inputs like text and time series data. Specifically, standard multi-head self-attention may fail to differentiate between intra-modality (e.g., within time series data) and cross-modality (e.g., between text and time series) interactions. This results in the blending of unrelated features from both modalities, causing the learned embeddings to lose modality-specific characteristics and leading to suboptimal performance. 

\textbf{Challenge III: How to effectively distill the knowledge to teach the student model?
} Traditional knowledge distillation methods often focus on transferring logits or soft labels from the teacher model to the student model, which primarily conveys coarse-grained information. While effective for tasks like classification, these approaches fail to capture the fine-grained relationships and contextual dependencies for regression like MTSF.

To address these challenges, we propose TimeKD, a novel framework that leverages a calibrated language model with privileged knowledge distillation to enable efficient and accurate MTSF. To bridge the domain gap between language and time series data, we design a cross-modality teacher model that integrates historical data and ground truth within a calibrated language model (CLM). This teacher model explicitly learns to map historical observations to future targets, mitigating the limitations of implicit mapping in conventional methods. To address the data entanglement problem, we introduce Subtractive Cross Attention (SCA), which isolates historical context and enriches the ground truth embeddings by filtering out irrelevant information from the privileged input. These enriched embeddings serve as robust privileged knowledge for guiding the student model. To ensure distillation efficiency, we devise correlation- and feature-based distillations that transfer the teacher’s privileged representations to a lightweight student model. This student model, which operates without LLM dependency during testing, retains the teacher's representational power while reducing computational cost, providing an efficient and scalable solution for real-world MTSF tasks.

% ========================================
% Paragraph 6
% Contribution
% 1. Substractive cross attention (Modality-Specific Attention Masking, last token for efficiency).
% 2. Correlation and Feature-based KD.
% 3. GT as input for privileged knowledge and no llm in testing for efficiency.
% ========================================

Our contributions are summarized as follows:
\begin{itemize}
    \item As far as we know, TimeKD is the first privileged knowledge distillation-based time series forecasting method.
    \item We devise a cross-modality reconstruction teacher network that is adapted from the calibrated language model, capable of learning generalizable representations from text to time series modality.
    \item We design the calibrated attention in the LLM (CLM) to enhance the intra-modality interactions for robust and time series representation. The CLM is distilled into a lightweight student model in the testing phase, which significantly accelerates inference speed.
    \item To enhance privileged information, we propose subtractive cross attention (SCA) to generate ground truth embeddings with historical context for efficient reconstruction and distillation.
    \item We develop correlation and feature distillations leveraging privileged information, enabling the student model to replicate the teacher's behavior while minimizing the output discrepancy between them.
\end{itemize}

The remainder of this paper is structured as follows. Section~\ref{sec:related_work} surveys related work. In Section~\ref{sec:problem}, we introduce preliminary definitions and define the problem of multivariate time series forecasting. The proposed TimeKD framework is detailed in Section~\ref{sec:method}, followed by experimental evaluations in Section~\ref{sec:exp}. Finally, Section~\ref{sec:conclusion} concludes the paper.

==> sections/sec1_intro_qianxiong.tex <==
\section{Introduction}
\label{sec:intro}

% ========================================
% Introduction flow
% P1 - background of MTSF, relationship with database
% P2 - different MTSF methods - challenges
% P3 - KD
% P4 - questions
% P5 - contributions
% ========================================


% P1 - background of MTSF, relationship with database
%Sensors play an important role in our daily lives~\cite{}, e.g., a large amount of loop detectors are installed to roads to sense traffic dynamics, 
The rapid revolution of sensing techniques and the proliferation of edge devices generate massive amounts of time series data~\cite{campos2023lightts,li2023towards,kieu2022anomaly}. % facilitating a variety of downstream applications, such as arrival time estimation~\cite{}, traffic prediction~\cite{}, and route planning~\cite{}. 
%Nevertheless, merely using existing sensor readings (i.e., those from historical and current timestamps) could hardly achieve these goals. 
It is important to extract useful knowledge from the historical time series data enabling a variety of time series-related applications, such as arrival time estimation~\cite{lin2023origin,tran2020deeptrans,yuan2020effective}, traffic prediction~\cite{liu2024spatial,fang2023spatio,yuan2021effective}, and route planning~\cite{xu2024managing,tian2023effective,luo2022diversified}. A fundamental aspect of such applications is multivariate time series forecasting (MTSF), which aims to predict future observations given historical observations~\cite{chang2024timedrl,zha2024scaling,shao2024exploring}. 
%Take route planning as an example, if traffic jams would shortly occur in a region, then detours should be planned to prevent people from driving to the affected roads, i.e., there exist demands to predict future sensor readings in advance.
%For this purpose, multivariate time series forecasting (MTSF)~\cite{zha2024scaling,chang2024timedrl,shao2024exploring} has been introduced to make accurate predictions for real-world applications, including but not limited to investment~\cite{zheng2024cross}, weather forecasting~\cite{fang2023spatio}, urban planning~\cite{sun2024urban}, and energy management~\cite{guo2024data}.

% P2 - different MTSF methods - challenges
Due to its significance, substantial research has been devoted to inventing effective MTSF models~\cite{DBLP:conf/kdd/LiangWNJ0SPW24}. 
Generally, existing MTSF methods can be categorized into classical methods~\cite{wu2023timesnet,Zeng2022AreTE,Yuqietal-2023-PatchTST,DBLP:journals/corr/abs-2310-06625} and large language model (LLM)-based methods~\cite{DBLP:conf/nips/ZhouNW0023, chang2023llm4ts,sun2023test,xue2023promptcast}.
Classical methods often adopt convolutional neural networks (CNNs)~\cite{wu2023timesnet}, fully-connected networks (FC)~\cite{Zeng2022AreTE}, and transformers~\cite{Yuqietal-2023-PatchTST} to learn spatial and temporal correlations across variables and time steps, respectively, for time series forecasting. %from historical time series, which are then leveraged to predict future time series.
However, the public benchmark datasets are often small-scale and fall short in diversity~\cite{liutimer}, \textit{hindering the usage of deeper layers (i.e., more parameters) and thus leading to shallow feature extraction.} %facilitate the learning of complex and robust forecasting knowledge}.
Recent studies~\cite{DBLP:conf/nips/ZhouNW0023, chang2023llm4ts,sun2023test,xue2023promptcast} apply large language models (LLMs) for time series forecasting inspired by the fact that time series and language data exhibit similar sequential format, as well as the powerful generic knowledge and knowledge transfer capabilities of LLMs. These methods often consider LLMs as powerful feature extractors to \textbf{extract robust representations from historical time series facilitating effective time series forecasting.} 
%Inspired by the fact that (1) time series and language data both belong to sequential data, and (2) LLMs, trained on abundant language data, have shown remarkable performance and generalizability in various tasks, some researchers~\cite{DBLP:conf/nips/ZhouNW0023, chang2023llm4ts,sun2023test,xue2023promptcast} have attempted to adapt LLMs for MTSF, 
%where the LLMs act as powerful feature extractors to \textbf{extract robust representations for historical time series}, making the forecasting relatively easier.

% P3 - KD
Unfortunately, due to the huge amount of parameters, the deployment of LLMs (e.g., LLaMA-7B~\cite{touvron2023llama}) would \textit{heavily slow down the inference speed}, posing challenges to support real-time functionalities in different applications.
Therefore, we propose to use knowledge distillation (KD)~\cite{gou2021knowledge} to distill the well-learned representation ability of LLM (teacher) to a classical model (student). In this way, the distilled model can not only \textbf{learn robust times series representations}, but also \textbf{enable fast inference}.
Nevertheless, it is not trivial to use KD, and several questions need to be considered and answered:
% Nevertheless, it is not trivial to develop LLMs-guided KD for multivariate time series forecasting due to the following challenges.

% P4 - questions
\noindent
\textbf{Q1: Which one should be distilled? Historical v.s. Future representations.}

\noindent
\textbf{A1: Future representations}.
Kindly remind that MTSF methods like iTransformer~\cite{DBLP:journals/corr/abs-2310-06625} will project the historical time series to \textit{shallow historical representations} via a linear layer. Then, some modules are leveraged to learn spatial and/or temporal correlations, while \textit{implicitly transform} the historical representations to \textbf{deep future representations}.
As KD should be conducted between same-type representations (i.e., distill teacher's historical/future representations to student's historical/future representations), KD can only be applied near either input or output ends, but not intermediate layers (due to the ambiguous intermediate status of representations).
Since shallow historical representations are obtained by few parameters, such parameter amount would be too small (for student model) to well mimic the knowledge of teacher model.
Therefore, KD should be applied between future representations.

\noindent
\textbf{Q2: How to obtain future time series representations in teacher model? Forecasting v.s. Reconstruction.}

\noindent
\textbf{A2: Reconstruction}.
There are roughly two ways for obtaining future times series representations:

\noindent
(1) Forecasting: Recall that \textit{LLMs essentially do not have good enough time series forecasting ability}~\cite{tan2024language}. Following existing works~\cite{DBLP:conf/nips/ZhouNW0023,jin2023time}, historical data is inputted to LLM, which is further fine-tuned on \textit{small-scale} time series datasets to acquire the forecasting ability, leading to \textit{inferior future representations}.

\noindent
(2) Reconstruction: Future data (i.e., ground truth labels) can be directly regarded as LLM's inputs to extract \textbf{superior future representations} (without learning new ability). Note that such way of taking labels as LLM's inputs is feasible with KD, as LLM is only used for distillation during training.

\noindent
\textbf{Q3: Can KD be further tailored for more effective MTSF?}

\noindent
\textbf{A3: Yes}. We present three modules, including \textbf{Prompt Construction (PC)} for better leveraging the intrinsic representation ability of LLM, \textbf{Representations Calibration (RC)} for calibrating future representations, and \textbf{Correlation-aware Knowledge Distillation (CKD)} for more fine-grained KD.

\noindent
(1) PC: As verified by existing works~\cite{}, wrapping historical time series as textual prompts appear to be a better choice than taking numerical time series as inputs. We attribute this to the fact that the trained LLMs cannot understand pure time series data, since there are no instructions inside. Therefore, we construct a prompt to input the future time series, as well as some contextual information like \textbf{\textit{xxx...}}, to LLM. Notably, the contextual information can \textbf{\textit{write some pros here...}}

\noindent
(2) RC: Note that the additional textual information is essential to LLM, yet redundant to our student model. Hence, we further design RC to purify the representations of the prompt, comprising two parts:
(a) We observe from empirical experiments (\textbf{\textit{Sec...}}) that too many textual representations will be fused into time series-related tokens, leading to entangled representations. Therefore, we dive into the attention layers of LLM, and equip them with a \textbf{Score Calibration (SC)} mechanism to \textbf{suppress the inter-modality fusion}, while \textbf{enhance the intra-modality correlations}, e.g., the attention scores between text and time series tokens would be biased with a negative value.
(b) After obtaining future representations from LLM, we further design a \textbf{Modality Separation (MS)} module to \textbf{remove the textual information doped in time series tokens}.
Consequently, the representations of time series tokens can be purer with the help of SC and MS, making it easier for KD.

\noindent
(3) CKD: \textbf{\textit{write some pros of correlation KD here...}}


% P5 - contributions
\textbf{\textit{To sum up...}}

The remainder of this paper is structured as follows. Section~\ref{sec:related_work} surveys related work. In Section~\ref{sec:problem}, we introduce preliminary definitions and define the problem of multivariate time series forecasting. The proposed TimeKD framework is detailed in Section~\ref{sec:method}, followed by experimental evaluations in Section~\ref{sec:exp}. Finally, Section~\ref{sec:conclusion} concludes the paper.
